Safe Importance Sampling in Model Predictive Path Integral Control

We introduce the notion of importance sampling under embedded barrier state control, titled Safety Controlled Model Predictive Path Integral Control (SC-MPPI). For robotic systems operating in an environment with multiple constraints, hard constraints are often encoded utilizing penalty functions when performing optimization. Alternative schemes utilizing optimization-based techniques, such as Control Barrier Functions, can be used as a safety filter to ensure the system does not violate the given hard constraints. In contrast, this work leverages the principle of a safety filter but applies it during forward sampling for Model Predictive Path Integral Control. The resulting set of forward samples can remain safe within the domain of the safety controller, increasing sample efficiency and allowing for improved exploration of the state space. We derive this controller through information theoretic principles analogous to Information Theoretic MPPI. We empirically demonstrate both superior sample efficiency, exploration, and system performance of SC-MPPI when compared to Model-Predictive Path Integral Control (MPPI) and Differential Dynamic Programming (DDP) optimizing the barrier state.

==> RSS 2023 Embedded Barrier States for Sampling-based MPC/commands.tex <==
% Base tex file for reusable commands

% Vector Variables
\newcommand{\vx}[0]{\mathbf{x}}
\newcommand{\vxb}[0]{\mathbf{\bar{x}}}
\newcommand{\vu}[0]{\mathbf{u}}
\newcommand{\vw}[0]{\mathbf{w}}
\newcommand{\vp}[0]{\mathbf{p}}
\newcommand{\vq}[0]{\mathbf{q}}
\newcommand{\vv}[0]{\mathbf{v}}
\newcommand{\vz}[0]{\mathbf{z}}
\newcommand{\vxdot}[0]{\dot{\vx}}
\newcommand{\ve}[0]{\mathbf{e}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\argmin}{\operatornamewithlimits{argmin}}


% Transpose
\newcommand{\rT}[0]{{\textrm{T}}}

% Trajectories
\newcommand{\xtraj}[0]{\mathbf{x}_{\tau}}
\newcommand{\xbtraj}[0]{\mathbf{\bar{x}}_{\tau}}
\newcommand{\utraj}[0]{\mathbf{u}_{\tau}}

% Domains
\newcommand{\real}[0]{\mathbb{R}}
\newcommand{\domain}[0]{\mathcal{D}}
\newcommand{\safeset}[0]{\mathcal{C}}

% Probability Distributions
\newcommand{\Pb}[0]{\mathbb{P}}
\newcommand{\Qb}[0]{\mathbb{Q}}
\newcommand{\gaussian}[2]{\mathcal{N}(#1, #2)}

% KL Divergence
\newcommand{\KL}[2]{\mathbb{KL}\left({#1}\parallel {#2}\right)}

% Expectation
\newcommand{\ExP}[2]{\mathbb{E}_{#1}\big[ #2 \big]}

% Math
\newcommand{\pluseq}{\mathrel{+}=}
\newcommand{\rd}[0]{\text{d}}


%% Acronyms
\begin{acronym}
\acro{MPPI}{Model-Predictive Path Integral Control}
\acro{Tube-MPPI}{Tube Model-Predictive Path Integral Control}
\acro{RMPPI}{Robust Model-Predictive Path Integral Control}
\acro{CCM}{Control Contraction Metrics}
\acro{MPC}{Model-Predictive Control}
\acro{IS}{Importance Sampling}
\acro{KL}{Kullback–Leibler}
\acro{GT-ARF}{Georgia Tech Autonomous Racing Facility}
\acro{iLQG}{iterative Linear Quadratic Gaussian}
\acro{AIS}{Augmented Importance Sampling}
\acro{SC-IS}{Safety-Controlled Importance Sampling}
\acro{CBFs}{Control Barrier Functions}
\acro{SC-MPPI}{Safety Controlled Model Predictive Path Integral Control}
\acro{BAS}{BArrier State}
\acro{DDP}{Differential Dynamic Programming}
\acro{MPC-DDP}{ Model Predictive Differential Dynamic Programming}
\acro{RMSE}{Root Mean-Squared Error}
\acro{DBaS}{Discrete Barrier States}
\end{acronym}

%% Editing commands
\newcommand{\edits}[1]{\textcolor{red}{#1}}
\newcommand{\needcite}[1]{\textcolor{blue}{#1}}


==> RSS 2023 Embedded Barrier States for Sampling-based MPC/packages.tex <==
% \usepackage{times}

% numbers option provides compact numerical references in the text. 
\usepackage{amsmath}
% \usepackage{amsthm}
\usepackage{amssymb}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{graphicx}
\usepackage{enumerate}
\usepackage{xcolor}
\usepackage{comment}
\usepackage{multicol}
\usepackage{hyperref}
\usepackage{tabularx}
\usepackage{makecell}
\usepackage{colortbl}
\usepackage{tablefootnote}
\usepackage{multirow}
\usepackage{paralist}
\usepackage{placeins}
\usepackage{nameref}
\usepackage{cancel}
\usepackage{subcaption}
\usepackage{multicol}
\usepackage[numbers]{natbib}
\def\bibfont{\footnotesize}  %\small %\footnotesize %\scriptsize
% Algorithms
\usepackage[ruled,vlined]{algorithm2e}
\usepackage[font=small]{caption}

\usepackage{float} % this is to force objects in places


% References
\usepackage{cleveref}

% Acronyms
\usepackage[nolist]{acronym}

% Figures
% \usepackage{subfig}

\renewcommand{\figureautorefname}{Fig.}

\newtheorem{condition}{Condition}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{proposition}[theorem]{Proposition}
\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    filecolor=magenta,      
    urlcolor=cyan,
}


% \hypersetup{
%     colorlinks=true,
%     linkcolor=blue,
%     filecolor=magenta,      
%     urlcolor=cyan,
% }
